On graph parameters guaranteeing fast Sandpile diffusion

The Abelian Sandpile Model is a discrete diffusion process defined on graphs (Dhar \cite{DD90}, Dhar et al. \cite{DD95}) which serves as the standard model of self-organized criticality. The transience class of a sandpile is defined as the maximum number of particles that can be added without making the system recurrent (\cite{BT05}). We demonstrate a class of sandpile which have polynomially bound transience classes by identifying key graph properties that play a role in the rapid diffusion process. These are the volume growth parameters, boundary regularity type properties and non-empty interior type constraints. This generalizes a previous result by Babai and Gorodezky (SODA 2007,\cite{LB07}), in which they establish polynomial bounds on $n \times n$ grid. Indeed the properties we show are based on ideas extracted from their proof as well as the continuous analogs in complex analysis. We conclude with a discussion on the notion of degeneracy and dimensions in graphs.

==> consFac.tex <==


In this section we will derive a constant factor approximation algorithm for single site particle addition transience classes. We later generalize it to multi site particle addition strategies. Using this, we will derive conditions required for a graph to satisfy the local superposition property.


% In \cite{CS11}, Choure and Vishwanathan demonstrate the following fact

Consider a sandpile $S = (V_{h} \cup \{s\}, E_{h}\cup \delta_{E} V_{h})$ with the sink node, $s$. If $x_{v}$ is the maximum number of particles that can be added at node $v$ without toppling the node $w$, then the following linear program bounds the value of $x$ from above.



\begin{eqnarray}
\text{max } x_{v} \nonumber \\
  0 \leq \sum_{v' \sim v} z(v') - \text{degree}(v).z(v)  + x_{v} & \leq & \text{degree(v)} - 1\nonumber \\
  \forall u \neq v : 0 \leq \sum_{u' \sim u} z(u') - \text{degree(u)}.z(u)  & \leq & \text{degree(u)} - 1\nonumber \\
  z(w) \leq 0, z \geq 0, x_{v} \geq 0  \nonumber
\end{eqnarray}

% The values of $x_{v}$ (the number of particles added at $v$) and $z$ (the vector of toppling counts) that are realized above are a feasible solution of this LP and hence the optimum of this LP yields an upper bound on the $R_{s}(v,w)$
Note that, in the program above and the ones to follow, the variables $v, w, \ldots$ all denote nodes from $V_{h}$. Similarly the summations indexed by nodes run over the vertices from $V_{h}$ only. The node $s$ is special, and whenever it figures, we will mention it explicitly. With the fixed sink node, $s$, we define $\pi_{w}(v)$ as the potential at node $v$ when a unit potential is applied (directly) at node $w$. In terms of these potential functions, the following bound holds. We give the proof here for completeness.

\begin{lem}(\cite{CS11})\label{lem:tclOptm} The optimum value of above LP is bounded from above by the following value,
 \begin{eqnarray}\label{equ:tclUpp}
\frac{1}{\pi_{w}(v)} \sum_{u}(\text{degree}(u)-1).\pi_{w}(u)
\end{eqnarray}
\end{lem}

\noindent \textbf{Proof:}  We consider the following relaxed version of the given LP.
\begin{eqnarray}
\text{max } x_{v} \nonumber \\
\sum_{v' \sim v} z(v') - \text{degree}(v).z(v)  + x_{v} & \leq & \text{degree}(v) - 1\nonumber \\
  \forall u \neq v :\sum_{u' \sim u} z(u') - \text{degree}(u).z(u)  & \leq & \text{degree}(u) - 1\nonumber \\
  z(w) \leq 0, z \geq 0, x_{v} \geq 0 \nonumber
\end{eqnarray}

From the weak duality for LPs, it follows that to obtain an upper bound of $\alpha$ on the optimum value of the above system, it suffices to find a feasible solution of the dual LP of value $\alpha$. The dual is the following :

\begin{eqnarray}
\text{min } \sum_{u}(\text{degree}(u)-1).Y(u)  \nonumber \\
\sum_{u' \sim w} Y(u') + Y' - \text{degree}(w).Y(w) & \geq & 0 \nonumber \\
\forall u \neq w : \sum_{u' \sim u} Y(u') - \text{degree}(u).Y(u) & \geq & 0 \nonumber \\
 Y(v) \geq 1, Y \geq 0, Y' \geq 0  \nonumber
\end{eqnarray}


Consider the following set of equations

\begin{eqnarray}
\sum_{u' \sim w} Y(u') + Y' - \text{degree}(w).Y(w) & = & 0  \label{equ:curInp} \\
\forall u \neq w : \sum_{u' \sim u} Y(u') -\text{degree}(u).Y(u) & = & 0 \\
Y(v)  & = & 1 \nonumber
\end{eqnarray}

A non-negative set of values satisfying the above set is feasible for the dual LP. We find these by considering the resistive circuit $\widehat{S}$, obtained by replacing each edge in $S$ by a unit resistance. We assign ground potential to the sink, and inject current at node $w$ such that it gets unit potential. The potential that develops on any node $u$ is $_{s}\pi_{w}(u)$. The potential value at node $v$, $\pi_{w}(v)$, can be used to scale the input current at $w$ thereby scaling all the potentials as well, such that potential at node $v$ becomes unit. It follows that the values $Y(u) = \pi_{w}(u)/\pi_{w}(v)$ and $Y'$ equaling the value of the current injected form a feasible solution of the dual LP. The objective value at this point is,

\begin{eqnarray}
\frac{1}{\pi_{w}(v)} \sum_{u}(\text{degree}(u)-1).\pi_{w}(u) \nonumber
\end{eqnarray}

\begin{flushright}$\square$ \end{flushright}



We will now argue that in the case of degree bound graphs, using some combinatorial properties of independent sets in sandpile graphs along with arguments similar to the ones outlined above for upper bound, one can derive tight (up to constant factors) lower bounds for the transience classes.

In the sandpile $S$, let $x_{v}'$ be the minimum number of particles that can need to be added at node $v$ such that the node $w$ topples at least once. Clearly $x_{v}' = x_{v} + 1$.  As in \cite{CS11}, the following LP relaxation forms a lower bound on the value of $x_{v}'$.

\begin{eqnarray}
\text{min } x_{v}' \nonumber \\
0 \leq \sum_{v' \sim v} z(v') - \text{degree}(v).z(v)  + x_{v} & \leq & \text{degree}(v) - 1\nonumber \\
  \forall u \neq v :0 \leq \sum_{u' \sim u} z(u') - \text{degree}(u).z(u)  & \leq & \text{degree}(u) - 1\nonumber \\
  z(w) \geq 1, z \geq 0, x_{v}' \geq 0 \nonumber
\end{eqnarray}

Consider the scenario in which we add $x_{v}'$ particles at $v$ and allow the configuration to settle down to stability. Furthermore, let the number of particles that appear at any node $u$ in the resulting stable configuration be $h_{u}$. The following lemma gives a lower bound on the particle count $x_{v}'$ in terms of these height functions $h_{u}$.

\begin{lem}\label{lem:tclLow} The value of the particle count $x_{v}'$ is bounded from below by the following value,
 \begin{eqnarray}\label{equ:tclLow}
\frac{1}{\pi_{w}(v)} \sum_{u} h(u).\pi_{w}(u)
\end{eqnarray}
\end{lem}


\noindent \textbf{Proof:} Clearly $0 \leq h_{u} \leq \text{degree}(u)$. In the linear program stated above, replacing each pair of constraints of the type  $0 \leq \sum_{v' \sim v} z(v') - d(v).z(v)  + x_{v}  \leq  d(v) - 1$ by $\sum_{v' \sim v} z(v') - d(v).z(v)  + x_{v} = h_{v} $, maintains the property that the optimum value is at least a lower bound to the \textit{exact} solution to the particle count $x_{v}'$. The altered LP is the following,

\begin{eqnarray}
\text{min } x_{v}' \nonumber \\
\sum_{v' \sim v} z(v') - \text{degree}(v).z(v)  + x_{v}' & = & h(v) \nonumber \\
  \forall u \neq v :\sum_{u' \sim u} z(u') - \text{degree}(u).z(u)  & = & h(u)\nonumber \\
  z(w) \geq 1, z \geq 0, x_{v}' \geq 0 \nonumber
\end{eqnarray}

To bound the optimum value, we will consider the dual of this minimization program and find a suitable feasible point. The value of the cost function at that point will be used as bound. The dual is the following maximization program.

\begin{eqnarray}
\text{max } Y' + \sum_{u} h(u).Y(u)  \nonumber \\
\sum_{u' \sim w} Y(u') + Y' - \text{degree}(w).Y(w) & \leq & 0 \nonumber \\
\forall u \neq w : \sum_{u' \sim u} Y(u') - \text{degree}(u).Y(u) & \leq & 0 \nonumber \\
 Y(v) \leq 1, Y \geq 0, Y' \geq 0  \nonumber
\end{eqnarray}

As in the previous lemma, we consider the following set of equations, whose feasible region is inside the one corresponding to the dual we mentioned above.

\begin{eqnarray}
\sum_{u' \sim w} Y(u') + Y' - d(w).Y(w) & = & 0  \nonumber \\
\forall u \neq w : \sum_{u' \sim u} Y(u') - \text{degree}(u).Y(u) & = & 0 \nonumber \\
Y(v)  & = & 1 \nonumber
\end{eqnarray}

A non-negative set of values satisfying the above set is feasible for the dual LP. We find these by considering the resistive circuit $\widehat{S}$ corresponding to the graph $S$ (with each edge having unit resistance). The sink node is assigned ground potential and just enough current is injected at node $w$ so that it attains unit potential. In terms of the standard potential functions described earlier, the potential that develops on any node $u$ is $_{s}\pi_{w}(u)$. The potential value at node $v$, $\pi_{w}(v)$, can be used to scale the input current at $w$ thereby scaling all the potentials as well, such that potential at node $v$ becomes unit. It follows that the values $Y(u) = \pi_{w}(u)/\pi_{w}(v)$ and $Y'$ equaling the value of the current injected form a feasible solution of the dual LP. The objective value at this point is,

\begin{eqnarray}
Y' + \frac{1}{\pi_{w}(v)} \sum_{u}h(u).\pi_{w}(u) \nonumber
\end{eqnarray}

Since the current, $Y'$, is a positive quantity, the above derivation implies the Lemma.$\square$

We will now show that the lower bound is at most a constant factor smaller then the upper bound. We start with defining an auxiliary set of variables $\hat{h}_{v}$ such that,

\begin{eqnarray}
\hat{h}_{v} = 1 \equiv h_{v} \geq 1 \nonumber
\end{eqnarray}

From the positivity of $\pi(.)$ function and the domination relation $\hat{h}_{v} \leq h_{v}$, the following inequality follows.

\begin{eqnarray}\label{equ:tclLower2}
\widehat{\Gamma} = \frac{1}{\pi_{w}(v)} \sum_{u}\hat{h}_{u}.\pi_{w}(u) \leq \frac{1}{\pi_{w}(v)} \sum_{u}h_{u}.\pi_{w}(u)
\end{eqnarray}

We will now bound the value $\widehat{\Gamma}$ from below.

\begin{lem}(Dhar \cite{DD06}, Babai and Gorodezky \cite{LB07})\label{lem:indSet} In any stable recurrent configuration, for every edge, both the incident vertices cannot have zero particles.\end{lem}

This follows from the fact that in any stable recurrent configuration, the last toppling of one of them would have taken place after the other and so the second node necessarily has at least one particle. For every edge $u,v$, at least one of $h_{u}$ and $h_{v}$ is $\geq 1$.

\begin{cor} The set of nodes $I = \{v : h_{v} = 0\}$ form an independent set.\end{cor}

Assume further that the graph satisfies ($\Delta$), i.e. the maximum degree is $\Delta$. Using this we will obtain the required bounds. Consider any vertex $v \in V_{h}$ along with its neighborhood (see figure (\ref{fig:localNei})). The function $\pi(.)$ is harmonic over this neighborhood, so we have

\begin{eqnarray}
 \text{degree}(v)\pi(v) = \sum_{u \sim v} \pi(u) \nonumber
\end{eqnarray}

from which we get the sum of $\pi(.)$ over any neighborhood in $V_{h}$ as,

\begin{eqnarray}
\pi(N(v)) = \pi(v) + \sum_{u \sim v} \pi(u) = (\text{degree}(v) + 1)\pi(v) \nonumber
\end{eqnarray}

The contribution of any local region in the restricted potential trace $\widehat{\Gamma}$ depends on just two possibilities regarding $h_{v}$. We deal with them separately.
 
%We distribute the measure associated with each node $v$ having non-zero height, $\pi(v)$, equally among itself and its neighborhood. So, $\pi(v)/2$ resides over $v$ and for any node $u \sim v$, $\pi(v)/2\text{degree}(v)$ resides with $u$. Note that this means that the total measure for any node $v$ is the sum of what it gets from each of its neighbors and what it has by itself.

\begin{itemize}
 \item[-] Case $h_{v} = 0$: $v \in I$, consequently none of its neighbors are in $I$. In this case the contribution to $\widehat{\Gamma}$ is the sum $\sum_{u \sim v}\pi(u) = \text{degree}(v)\pi(v) = \frac{\text{degree}(v)}{\text{degree}(v) + 1}\pi(N(v))$.

 \item[-] Case $h_{v} = 1$: $v \notin I$, and some of its neighbors are in $I$. Assume the worst case scenario when all the neighbors are in $I$. The contribution to $\widehat{\Gamma}$ in such a situation is just $\pi(v) = \frac{1}{\text{degree}(v) + 1}\pi(N(v))$.
\end{itemize}


%\begin{itemize}
% \item[-] Case $h_{v} = 0$: $v \in I$, consequently none of its neighbors are in $I$. In this case the contribution to $\widehat{\Gamma}$ is the sum $\sum_{u \sim v}\pi(u) = \text{degree}(v)\pi(v) = \frac{\text{degree}(v)}{\text{degree}(v) + 1}\pi(N(v))$.
%
% \item[-] Case $h_{v} = 1$: $v \notin I$, and some of its neighbors are in $I$. Assume the worst case scenario when all the neighbors are in $I$. The contribution to $\widehat{\Gamma}$ in such a situation is just $\pi(v) = \frac{1}{\text{degree}(v) + 1}\pi(N(v))$.
%\end{itemize}


\begin{figure}[ht]
\centering
\includegraphics[width=.5\textwidth]{figures/localNei.jpeg}
\caption{Neighborhood around vertex $v$; two cases, $v$ selected and not selected in $I$}
\label{fig:localNei}
\end{figure}

It follows that any neighborhood $N(v)$ contributes at least $\frac{1}{\text{degree}(v) + 1}\pi(N(v))$ to $\widehat{\Gamma}$, regardless of the specific values of $h_{v}$. Since the degree is bounded by $\Delta$, this translates to a minimum contribution of $\frac{1}{\Delta + 1}\pi(N(v))$. Therefore, the value of $\widehat{\Gamma}$ in equation (\ref{equ:tclLower2}), for any independent set $I$, is at least

\begin{eqnarray} \label{equ:tclLower}
\frac{1}{(\Delta + 1)\pi_{w}(v)} \sum_{u}\pi_{w}(u)
\end{eqnarray}

The upper bound yielded by Lemma \ref{lem:tclOptm} is bounded from above by,

\begin{eqnarray} \label{equ:tclUpper}
\frac{(\Delta - 1)}{\pi_{w}(v)} \sum_{u}\pi_{w}(u)
\end{eqnarray}

Using equations (\ref{equ:tclUpper}) and (\ref{equ:tclLower}), we obtain the following two sided bounds for degree bounded graphs,

\begin{eqnarray} \label{equ:tclSandW}
\frac{1}{(\Delta + 1)\pi_{w}(v)} \sum_{u}\pi_{w}(u) \leq x_{v} \leq \frac{(\Delta - 1)}{\pi_{w}(v)} \sum_{u}\pi_{w}(u)
\end{eqnarray}

\begin{thm}\label{thm:consFac} For any sandpile with bounded vertex degrees, the minimum number of particles that need to be added at any vertex $v$ to observe a toppling at any vertex $w$ is equal, up to constant factors, to the following expression,
\begin{eqnarray}
\frac{1}{\pi_{w}(v)} \sum_{u}\pi_{w}(u)
\end{eqnarray}
\end{thm}

The computation of transience class $\text{tcl}(S)$ requires evaluating the above expression for all possible combinations of $v, w \in V(S)$. Computing the function $\pi(.)$ can be done in very efficiently following the recent path breaking work by \cite{KMP-1}, \cite{KMP-2}, \cite{ST} on solving symmetric, diagonally, dominant linear systems. Consequently, finding the pair with worst estimates is also easy to do.

\begin{cor} There exists a polynomial time algorithm which computes the transience class of a degree bound sandpile up to constant factors. \end{cor}

This answers one of the main questions raised in \cite{CS11}. In this paper, the authors also derived several sandpile properties in analogy with the electric network theory. However, because of one sided bounds, most of these were also one sided. The sandwich bounds we have derived in this section will imply tighter versions for several of those potential theoretic properties for sandpile.




